Continuous emission ultrasound: a new paradigm to ultrafast ultrasound imaging

Current imaging techniques in echography rely on the pulse-echo (PE) paradigm which provides a straight-forward access to the in-depth structure of tissues. They inherently face two major challenges: the limitation of the pulse repetition frequency, directly linked to the imaging framerate, and, due to the emission scheme, their blindness to the phenomena that happen in the medium during the majority of the acquisition time. To overcome these limitations, we propose a new paradigm for ultrasound imaging, denoted by continuous emission ultrasound imaging (CUEI) \cite{CEUIpatent2023}, for a single input single output (SISO) device. A continuous insonification of the medium is done by the probe using a coded waveform inspired from the radar and sonar literature. A framework coupling a sliding window approach (SWA) and pulse compression methods processes the recorded echoes to rebuild a motion-mode (M-mode) image from the medium with a high temporal resolution compared to state-of-the-art ultrafast imaging methods. A study on realistic simulated data, with regards to the motion of the medium, has been carried out and, achieved results assess an unequivocal improvement of the slow time frequency up to, at least, two orders of magnitude compared to ultrafast US imaging methods. This enhancement leads, therefore, to a ten times improvement in the temporal separability of the imaging system. In addition, it demonstrates the capability of CEUI to catch relatively short and quick events, in comparison to the imaging period of PE methods, at any instant of the acquisition.

==> TXT/txt_discussion/discussion_contribution.tex <==
% SYNTHESIS OF FINDINGS: 
%
% The discussion section allows authors to synthesize the information presented in the results section. This involves drawing conclusions based on the data and explaining how these conclusions align with the study's objectives.
%
% CONTRIBUTION TO THE FIELD: 
%
% Authors use the discussion section to highlight the novel aspects of their work and articulate how their study contributes to the existing body of knowledge. This may include proposing new hypotheses, suggesting alternative explanations, or identifying gaps in current understanding.

% IMPROVEMENT OF IMAGING FRAMERATE
%


%
% CUI f_img != f_s
% In practice, the true imaging framerate of CUI is limited by as much by the sampling frequency of the probe which minors the temporal step between two successive windows $w$ and $w+1$ in the SWA as by the size of the reference signal $N_E$ which defines indirectly the temporal scale of dynamic phenomenons we aim at imaging. Indeed, in our case, the step chosen equals to $\frac{N_E}{4} \sim 1.66 \mu s$ is too small with regards to the dynamic of the 2 simulated media and can be increase in order to reduce the post-processing computational cost.

==> TXT/txt_results/results_decoding.tex <==
\subsection{Decoding filter comparison}\label{subsec_filter_evaluation}

% Objective
The decoding method impacts significantly the image reconstruction quality. Before evaluating the robustness of CUI to fast and quick events, let compare the performances of each decoding scheme described in the subsection \ref{subsec_decoding}. 
%
% Method of comparison
To do so, motion-mode images are reconstructed using the CUI approach introduced in the subsection \ref{subsec_emission_reception_scheme} on the same simulated ultrasound data, but with distincts decoding methods: the matched filter (MF), the ISLR mismatched filter (ISLR mMF) (\textbf{REF}), and the ISLR mMF with a constraint relaxation on the mainlobe width and with and extended PSF (wide ISLR mMF).   

The results are represented on the Figure \ref{fig_comparison_filter}: the performance  will be assessed using the ISLR (integrated SideLobe Ratio), THE PSLR (Peak SideLobe Ratio) and the MLW (MainLobe Width) at -3dB. 

The global performances using the MF and the ISLR mMF are quit the same: the average background or estimation noise due to the sidelobes of the PSF and cross-talks between each reference signal $\mathbf{x}_w$ and the other parts of the emitted waveform contained in its associated windowed recorded echoes signal $\mathbf{y}_w$.

\begin{figure*}%[H]
    \centering
    \includegraphics[width=0.95\textwidth]{IMG/RESULTS/comparison_filter_v4_colorbar.png}
    \captionsetup{justification=centering}
    \caption{Motion-Mode images of a medium containing a single scatterer moving at $2 \; m.s^{-1}$ on $[110,540] \mu s$. The images are obtained using the CUI approach whith different decoding filters: the MF in red, the ISLR mMF in green, the wide PSF ISLR mMF in blue. The graphs on the first two lines display the ISLR and the PSLR for each frame of the 3 motion-mode images. The vertical graphs display for each imaged depth, the mean magnitude over all frames.}
    \label{fig_comparison_filter}
\end{figure*}

for $N_E=1001 samp$ : mainlobe = $1.41 \lambda$ $0.71 \lambda$ $0.63 \lambda$
dilatation of the mainlobe width due to the velocity of the scatterer

for $N_E=401 samp$ : mainlobe = $1.40 \lambda$ $0.67 \lambda$ $0.67 \lambda$ 
% ATTENTION HYPER-PARAMETRE 

==> TXT/txt_results/results_multiTarget.tex <==
\subsection{Multi-target performances}
%
\begin{figure}[H]\label{fig_mmode_2scat}
    \centering
    \includegraphics[width=0.45\textwidth]{IMG/RESULTS/2scats_uniform_v1.png}
    \captionsetup{justification=centering}
    \caption{Motion-Mode images of a medium containing 2 closed scatterers: one is remaining static at a range of 30.5 mm, the second is distant from 30 mm at the beginning and moves away at a constant axial speed equals to $2 \; m.s^{-1}$.}
\end{figure}

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{IMG/RESULTS/oscillation_v2.png}}]{First A. Author} biography
\end{IEEEbiography}
